HistRED: A Historical Document-Level Relation Extraction Dataset

Despite the extensive applications of relation extraction (RE) tasks in various domains, little has been explored in the historical context, which contains promising data across hundreds and thousands of years. To promote the historical RE research, we present HistRED constructed from Yeonhaengnok. Yeonhaengnok is a collection of records originally written in Hanja, the classical Chinese writing, which has later been translated into Korean. HistRED provides bilingual annotations such that RE can be performed on Korean and Hanja texts. In addition, HistRED supports various self-contained subtexts with different lengths, from a sentence level to a document level, supporting diverse context settings for researchers to evaluate the robustness of their RE models. To demonstrate the usefulness of our dataset, we propose a bilingual RE model that leverages both Korean and Hanja contexts to predict relations between entities. Our model outperforms monolingual baselines on HistRED, showing that employing multiple language contexts supplements the RE predictions. The dataset is publicly available at: https://huggingface.co/datasets/Soyoung/HistRED under CC BY-NC-ND 4.0 license.

==> table/ablation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t]
\centering
\resizebox{0.9\columnwidth}{!}{%
\begin{tabular}{l|lll}
\toprule
Model & \textit{SL}=0 & \textit{SL}=1 & \textit{SL}=2 \\ \midrule
Final Model & \textbf{62.43} & \textbf{59.10} & \textbf{52.92} \\
Joint FCN + add & {\ul 61.44} & 57.39 & 50.77 \\
Joint FCN + concat & 58.97 & {\ul 59.00} & {\ul 52.85} \\
\bottomrule
\end{tabular}%
}
\caption{Analysis of different prediction layer types. }
\label{tab:ablation_study}
\end{table}

==> table/table_ent_re_types.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \begin{table}[h]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|l|l|}
% \hline
% \rowcolor[HTML]{C0C0C0} 
% \multicolumn{1}{|c|}{\cellcolor[HTML]{C0C0C0}\textbf{Entity Types}} &
%   \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\textbf{Relation Types}} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Location, Person, Number, \\ Product, Datetime, Organization, \\ Food, Book, Clothes, Others\end{tabular} &
%   \begin{tabular}[c]{@{}l@{}}Nearby, Alternate\_name,\\ Per:position\_held, Per:country\_of\_citizenship, \\ Per:worn\_by, Per:place\_of\_residence,\\ Per:other\_family, Per:child, Per:sibling, \\ Per:friend, Per:enemy,\\ Per:place\_of\_birth, Per:place\_of\_death, \\ Per:date\_of\_birth, Per:date\_of\_death,\\ Loc:functions\_as, Loc:famous\_for, \\ Org:member\_of, Product:provided\_by, \\ Others\end{tabular} \\ \hline
% \end{tabular}%
% }
% \caption{\textbf{Types of Entity and Relation}. We construct 10 entity and 20 relation types, when each of them includes others.}
% \label{tab:ent_re_types}
% \end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






\begin{table*}[t]
\center
\begin{tabular}{@{}ll@{}}
\toprule
Entity   & Location, Person, Number, Product, Book, Clothes, Datetime, Organization, Food, Others  \\ \midrule
Relation & \begin{tabular}[c]{@{}l@{}}Nearby, Alternative\_name, Per:wone\_by, Per:position\_held, Per:country\_of\_cityzenship,\\ Per:place\_of\_residence, Per:other\_family, Per:child, Per:sibling, Per:friend, Per:enemy,\\ Per:place\_of\_birth, Per:place\_of\_death, Per:date\_of\_birth, Per:date\_of\_death,\\ Loc:function\_as, Loc:famous\_for, Org:member\_of, Product:provided\_by, Others\end{tabular} \\ \bottomrule
\end{tabular}
\caption{\sy{단일 컬럼으로 사이즈 줄여보기. section 2.1 위에 들어가도록} Types of entity and relation. We define 10 entity and 20 relation types, when each of them includes `others'.}
\label{tab:ent_re_types}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{table*}[t]
% \center
% \begin{tabular}{@{}ll@{}}
% \toprule
% \multicolumn{1}{c}{} & \multicolumn{1}{c}{Type}                                                                                                                                                                                                                                                                                                                                                                                   \\ \midrule
% Entity               & Location., Person, Number, Product, Book, Clothes, Datetime, Organization, Food, Others                                                                                                                                                                                                                                                                                                                    \\
% Relation             & \begin{tabular}[c]{@{}l@{}}Nearby, Alternative\_name, Per:wone\_by, Per:position\_held, Per:country\_of\_cityzenship,\\ Per:place\_of\_residence, Per:other\_family, Per:child, Per:sibling, Per:friend, Per:enemy,\\ Per:place\_of\_birth, Per:place\_of\_death, Per:date\_of\_birth, Per:date\_of\_death,\\ Loc:function\_as, Loc:famous\_for, Org:member\_of, Product:provided\_by, Others\end{tabular} \\ \bottomrule
% \end{tabular}
% \caption{Types of entity and relation. We define 10 entity and 20 relation types, when each of them includes others.}
% \label{tab:ent_re_types}
% \end{table*}
